If it Looks like a Human and Speaks like a Human ... Dialogue and cooperation in human-robot interactions

The paper presents the results of a behavioral experiment conducted between February 2020 and March 2021 at Universit\`a Cattolica del Sacro Cuore, Milan Campus in which students were matched to either a human or a humanoid robotic partner to play an iterated Prisoner's Dilemma. The results of a Logit estimation procedure show that subjects are more likely to cooperate with human rather robotic partners; that are more likely to cooperate after receiving a dialogic verbal reaction following the realization of a sub-obtimal social outcome; that the effect of the verbal reaction is independent on the nature of the partner. Our findings provide new evidence on the effect of verbal communication in strategic frameworks. Results are robust to the exclusion of students of Economics related subjects, to the inclusion of a set of psychological and behavioral controls, to the way subjects perceive robots' behavior and to potential gender biases in human-human interactions.

==> OLS/OLSreaction_interactionCV.tex <==
                    &   \multicolumn{2}{c}{Benchmark}           &\multicolumn{2}{c}{Including Choice at Stage 1} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
Choice: ``Cooperate'' &   Full sample   &Excl. failed tests\tnote{$\dagger$}    &   Full sample   &Excl. failed tests\tnote{$\dagger$}    \\
\midrule
DVR$\times$Robot&      0.0474   &      0.0953   &      0.0245   &      0.0775   \\
            &     (0.121)   &     (0.129)   &     (0.117)   &     (0.124)   \\
            &               &               &               &               \\
DVR    &       0.179   &       0.158   &       0.178   &       0.150   \\
            &    (0.084)** &    (0.093)*  &    (0.083)** &    (0.090)*  \\
            &               &               &               &               \\
Robot       &      -0.152   &      -0.199   &      -0.166   &      -0.221   \\
            &    (0.088)*  &    (0.093)** &    (0.086)*  &    (0.092)** \\
            &               &               &               &               \\
Cooperate (Stage 1)&               &               &       0.276   &       0.290   \\
            &               &               &    (0.061)***&    (0.065)***\\
            &               &               &               &               \\
Controls    &         Yes   &         Yes   &         Yes   &         Yes   \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   \\
Wave                &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Adj. R-sq.  &        0.05   &        0.06   &        0.11   &        0.13   \\
Obs         &         305   &         268   &         305   &         268   \\
LL          &        -200   &        -174   &        -190   &        -164   \\
AIC         &         441   &         387   &         422   &         367   \\
BIC         &         515   &         455   &         500   &         439   \\

==> OLS/OLSreaction_interactionCV_allest.tex <==
                    &   \multicolumn{2}{c}{Benchmark}           &\multicolumn{2}{c}{Including Choice at Stage 1} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
Choice: ``Cooperate'' &   Full sample   &Excl. failed tests\tnote{$\dagger$}    &   Full sample   &Excl. failed tests\tnote{$\dagger$}    \\
\midrule
DVR$\times$Robot    &      0.0474   &      0.0953   &      0.0245   &      0.0775   \\
                    &     (0.121)   &     (0.129)   &     (0.117)   &     (0.124)   \\
                    &               &               &               &               \\
DVR                 &       0.179   &       0.158   &       0.178   &       0.150   \\
                    &    (0.084)** &    (0.093)*  &    (0.083)** &    (0.090)*  \\
                    &               &               &               &               \\
Robot               &      -0.152   &      -0.199   &      -0.166   &      -0.221   \\
                    &    (0.088)*  &    (0.093)** &    (0.086)*  &    (0.092)** \\
                    &               &               &               &               \\
Female              &     -0.011   &      0.011  &     -0.020   &    -0.004   \\
                    &    (0.064)   &    (0.068)   &    (0.062)   &    (0.066)   \\
                    &               &               &               &               \\
Freshman            &     0.003   &     -0.072   &     0.006   &     -0.062   \\
                    &    (0.080)   &    (0.083)   &    (0.080)   &    (0.082)   \\
                    &               &               &               &               \\
Economics           &     -0.074   &     -0.080   &     -0.040   &     -0.037   \\
                    &    (0.062)   &    (0.065)   &    (0.061)   &    (0.064)   \\
                    &               &               &               &               \\
Test failed         &      0.079   &              &      0.022   &              \\
                    &    (0.088)   &           &    (0.088)   &            \\
                    &               &               &               &               \\
Cooperate (Stage 1) &               &               &       0.276   &       0.290   \\
                    &               &               &    (0.061)***&    (0.065)***\\
                    &               &               &               &               \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   \\
Wave                &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Adj. R-sq.          &        0.05   &        0.06   &        0.11   &        0.13   \\
Obs                 &         305   &         268   &         305   &         268   \\
LL                  &        -200   &        -174   &        -190   &        -164   \\
AIC                 &         441   &         387   &         422   &         367   \\
BIC                 &         515   &         455   &         500   &         439   \\


==> OLS/OLSrobot_DVR_CV.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &   Benchmark   &               &Including Choice at Stage 1   &               \\
Choice: 'Cooperate' &   Benchmark   &Excl. failed tests   &   Benchmark   &Excl. failed tests   \\
                    &   b/se/r\_se   &   b/se/r\_se   &   b/se/r\_se   &   b/se/r\_se   \\
\midrule
treat               &     -0.0587   &     -0.0617   &      -0.115   &      -0.129   \\
                    &    (0.0892)   &    (0.0936)   &    (0.0859)   &    (0.0881)   \\
                    &               &               &               &               \\
Experimental wave=0 &           0   &           0   &           0   &           0   \\
                    &         (.)   &         (.)   &         (.)   &         (.)   \\
                    &               &               &               &               \\
Experimental wave=1 &     -0.0303   &     -0.0172   &     -0.0586   &     -0.0538   \\
                    &    (0.0904)   &    (0.0912)   &    (0.0934)   &    (0.0933)   \\
                    &               &               &               &               \\
Cooperate (Stage 1) &               &               &       0.350   &       0.409   \\
                    &               &               &    (0.0881)***&    (0.0920)***\\
                    &               &               &               &               \\
Controls            &         Yes   &         Yes   &         Yes   &         Yes   \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Adj. R-sq.          &        0.00   &        0.03   &        0.10   &        0.17   \\
Obs                 &         157   &         141   &         157   &         141   \\
LL                  &         -94   &         -82   &         -85   &         -71   \\
AIC                 &         224   &         199   &         207   &         177   \\
BIC                 &         279   &         249   &         265   &         230   \\
\bottomrule
\end{tabular}
}


==> OLS/OLSrobot_noDVR_CV.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &   Benchmark   &               &Including Choice at Stage 1   &               \\
Choice: 'Cooperate' &   Benchmark   &Excl. failed tests   &   Benchmark   &Excl. failed tests   \\
                    &   b/se/r\_se   &   b/se/r\_se   &   b/se/r\_se   &   b/se/r\_se   \\
\midrule
Robot               &      -0.142   &      -0.191   &      -0.151   &      -0.207   \\
                    &    (0.0971)   &     (0.101)*  &    (0.0958)   &    (0.0992)** \\
                    &               &               &               &               \\
Experimental wave=0 &           0   &           0   &           0   &           0   \\
                    &         (.)   &         (.)   &         (.)   &         (.)   \\
                    &               &               &               &               \\
Experimental wave=1 &       0.166   &       0.203   &       0.166   &       0.190   \\
                    &    (0.0964)*  &     (0.105)*  &    (0.0939)*  &     (0.102)*  \\
                    &               &               &               &               \\
Cooperate (Stage 1) &               &               &       0.234   &       0.215   \\
                    &               &               &    (0.0948)** &     (0.102)** \\
                    &               &               &               &               \\
Controls            &         Yes   &         Yes   &         Yes   &         Yes   \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Adj. R-sq.          &        0.00   &        0.01   &        0.04   &        0.04   \\
Obs                 &         148   &         127   &         148   &         127   \\
LL                  &         -98   &         -83   &         -94   &         -80   \\
AIC                 &         232   &         199   &         227   &         196   \\
BIC                 &         286   &         248   &         284   &         247   \\
\bottomrule
\end{tabular}
}


==> desc_stimulus.tex <==
\textbf{Observed outcome}    & \textbf{DVR type performed by partner} \\
(Subject, Partner)  & \\ \midrule
(C, N)                              & Apology \\
(N, C)                              & Reprimand    \\
(N, N)                              & Disappointment\\
(C, C)                              & None          \\

==> resdesign.tex <==
Experimental Condition  & Stimulus & No Stimulus \\ 
 Human                  & cell5 & cell6 \\ 
 Robot                  & cell8 & cell9 \\ 


==> tab_control_economics.tex <==
                  &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   &\multicolumn{1}{c}{(3)}   \\
  &       Logit   &          OR   &     Margins   \\
\midrule
Robot$\times$Economics&      -0.011   &       0.989   &      -0.003   \\
                    &     (0.818)   &     (0.809)   &     (0.189)   \\
                    &     [0.989]   &     [0.989]   &     [0.989]   \\
Partner=Robot       &      -0.739   &       0.477   &      -0.171   \\
                    &     (0.508)   &     (0.242)   &     (0.117)   \\
                    &     [0.145]   &     [0.145]   &     [0.144]   \\
Economics           &      -0.875   &       0.417   &      -0.202   \\
                    &     (0.670)   &     (0.279)   &     (0.154)   \\
                    &     [0.192]   &     [0.192]   &     [0.191]   \\
Cooperate (Stage 1) &       2.028***&       7.602***&       0.468***\\
                    &     (0.658)   &     (4.998)   &     (0.155)   \\
                    &     [0.002]   &     [0.002]   &     [0.003]   \\
Constant            &       0.625   &       1.868   &               \\
                    &     (0.967)   &     (1.806)   &               \\
                    &     [0.518]   &     [0.518]   &               \\
                    \midrule
Controls            &         Yes   &         Yes   &         Yes   \\
Inst. order         &         Yes   &         Yes   &         Yes   \\
\midrule
Obs                 &         153   &         153   &         153   \\
Pseudo R-sq.        & \multicolumn{2}{c}{0.14}      &           .   \\
LL                  & \multicolumn{2}{c}{-86}       &           .    \\
AIC                 & \multicolumn{2}{c}{195}       &           .   \\
BIC                 & \multicolumn{2}{c}{228}       &           .   \\


==> tab_humVSrobotCV.tex <==
\textbf{No DVR condition} &&&&&& \\  
                    &   \multicolumn{3}{c}{Benchmark}           &\multicolumn{3}{c}{Including Choice at Stage 1} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
Choice: ``Cooperate'' &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   \\
\midrule
Robot               &      -0.640   &      -0.855   &      -0.159   &      -0.705   &      -0.957   &      -0.175   \\
                    &     (0.395)   &     (0.419)** &    (0.098)   &     (0.405)*  &     (0.430)** &     (0.101)*  \\
                    &               &               &               &               &               &               \\
Cooperate (Stage 1) &               &               &               &       1.146   &       1.037   &       0.285   \\
                    &               &               &               &     (0.444)***&     (0.466)** &     (0.110)***\\
                    &               &               &               &               &               &               \\
Controls            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Wave         &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Pseudo R-sq.        &        0.09   &        0.10   &               &        0.13   &        0.13   &               \\
Obs                 &         148   &         127   &         148   &         148   &         127   &         148   \\
LL                  &         -93   &         -79   &               &         -89   &         -76   &               \\
AIC                 &         222   &         191   &              &         217   &         188   &            \\
BIC                 &         276   &        240   &             &         274   &         239   &             \\\midrule
\textbf{DVR condition} &&&&&& \\
                    &   \multicolumn{3}{c}{Benchmark}           &\multicolumn{3}{c}{Including Choice at Stage 1} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
Choice: 'Cooperate' &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   \\
\midrule
Robot               &      -0.297   &      -0.290   &     -0.062   &      -0.676   &      -0.789   &      -0.135   \\
                    &     (0.406)   &     (0.445)   &    (0.085)   &     (0.450)   &     (0.508)   &    (0.090)   \\
                    &               &               &               &               &               &               \\
Cooperate (Stage 1) &               &               &               &       1.859   &       2.389   &       0.372   \\
                    &               &               &               &     (0.476)***&     (0.566)***&    (0.0936)***\\
                    &               &               &               &               &               &               \\
Controls            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Wave         &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Pseudo R-sq.        &        0.09   &        0.12   &               &        0.18   &        0.24   &               \\
Obs                 &         157   &         141   &         157   &         157   &         141   &         157   \\
LL                  &         -89   &         -78   &               &         -81   &         -67   &               \\
AIC                 &         215   &         191   &          &         199   &         171   &             \\
BIC                 &         270   &         241   &          &         258   &         224   &             \\

==> tab_reaction_byADAPTIVE.tex <==
\multicolumn{3}{l}{\textbf{Robot's behavior perceived as Adaptive}} &&&& \\  
                    &   \multicolumn{3}{c}{Benchmark}           &\multicolumn{3}{c}{Including Choice at Stage 1} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
Choice: ``Cooperate'' &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   \\
\midrule
DVR$\times$Robot          &      -0.961   &      -0.786   &      -0.228   &      -1.442   &      -1.126   &      -0.341   \\
                    &     (0.843)   &     (0.935)   &     (0.200)   &     (0.897)   &     (0.985)   &     (0.212)   \\
                    &               &               &               &               &               &               \\
DVR                 &       1.222   &       1.119   &       0.291   &       1.480   &       1.258   &       0.350   \\
                    &     (0.616)** &     (0.702)   &     (0.146)** &     (0.657)** &     (0.742)*  &     (0.155)** \\
                    &               &               &               &               &               &               \\
Robot               &       0.133   &      -0.113   &      0.032   &       0.101   &      -0.301   &      0.024   \\
                    &     (0.600)   &     (0.666)   &     (0.143)   &     (0.627)   &     (0.705)   &     (0.148)   \\
                    &               &               &               &               &               &               \\
Cooperate (Stage 1) &               &               &               &       1.446   &       1.388   &       0.342   \\
                    &               &               &               &     (0.513)***&     (0.528)***&     (0.121)***\\
                    &               &               &               &               &               &               \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Wave            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Pseudo R-sq.        &        0.13   &        0.13   &               &        0.18   &        0.18   &               \\
Obs                 &         125   &         110   &         125   &         125   &         110   &         125   \\
LL                  &         -74   &         -65   &               &         -70   &         -62   &               \\
AIC                 &         180   &         163   &             &         173   &         157   &             \\
BIC                 &         225   &         206   &             &         222   &         203   &             \\
\midrule
\multicolumn{3}{l}{\textbf{Robot's behavior perceived as Pre-determined by an algorithm}} &&&& \\  
                    &   \multicolumn{3}{c}{Benchmark}           &\multicolumn{3}{c}{Including Choice at Stage 1} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
Choice: 'Cooperate' &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   \\
\midrule
DVR$\times$Robot         &       0.533   &       0.897   &       0.129   &       0.569   &       0.880   &       0.138   \\
                    &     (0.690)   &     (0.756)   &     (0.168)   &     (0.728)   &     (0.803)   &     (0.177)   \\
                    &               &               &               &               &               &               \\
DVR                 &       0.884   &       0.747   &       0.214   &       0.901   &       0.795   &       0.218   \\
                    &     (0.489)*  &     (0.537)   &     (0.118)*  &     (0.512)*  &     (0.567)   &     (0.124)*  \\
                    &               &               &               &               &               &               \\
Robot               &      -1.178   &      -1.509   &      -0.286   &      -1.275   &      -1.656   &      -0.309   \\
                    &     (0.494)** &     (0.551)***&     (0.120)** &     (0.527)** &     (0.597)***&     (0.128)** \\
                    &               &               &               &               &               &               \\
Cooperate (Stage 1) &               &               &               &       1.729   &       1.922   &       0.419   \\
                    &               &               &               &     (0.410)***&     (0.465)***&    (0.010)***\\
                    &               &               &               &               &               &               \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Wave            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Pseudo R-sq.        &        0.13   &        0.15   &               &        0.21   &        0.24   &               \\
Obs                 &         180   &         158   &         180   &         180   &         158   &         180   \\
LL                  &        -107   &         -91   &               &         -97   &         -82   &               \\
AIC                 &         246   &         215   &             &         229   &         197   &             \\
BIC                 &         297   &         264   &             &         283   &         249   &            \\

==> tab_reaction_psycho.tex <==
                    &   \multicolumn{3}{c}{Benchmark}           &\multicolumn{3}{c}{Including Choice at Stage 1} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
Choice: ``Cooperate'' &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   &   Full sample   &Excl. failed tests\tnote{$\dagger$}   &     Margins   \\
\midrule
DVR$\times$Robot    &       0.162   &       0.349   &      0.0393   &      0.0248   &       0.266   &     0.006   \\
                    &     (0.509)   &     (0.551)   &     (0.123)   &     (0.529)   &     (0.574)   &     (0.128)   \\
                    &               &               &               &               &               &               \\
DVR                 &       0.836   &       0.751   &       0.202   &       0.913   &       0.781   &       0.220   \\
                    &     (0.366)** &     (0.404)*  &    (0.0883)** &     (0.381)** &     (0.422)*  &    (0.0915)** \\
                    &               &               &               &               &               &               \\
Robot               &      -0.715   &      -0.912   &      -0.173   &      -0.787   &      -1.070   &      -0.190   \\
                    &     (0.359)** &     (0.389)** &    (0.0871)** &     (0.373)** &     (0.409)***&    (0.090)** \\
                    &               &               &               &               &               &               \\
Cooperate (Stage 1) &               &               &               &       1.305   &       1.415   &       0.315   \\
                    &               &               &               &     (0.289)***&     (0.314)***&    (0.070)***\\
                    &               &               &               &               &               &               \\
\textit{Psychological and behavioral controls:} &&&&&& \\
Risk scale			&     0.006   	&     0.008   	&     0.001   	&     -0.013   	&    -0.009   &    -0.003  \\
                    &    (0.060)   	&    (0.062)   	&    (0.014)   	&    (0.061)   	&    (0.065)   &    (0.015)   \\
                    &               &               &               &               &               &               \\
Trust scale         &       0.222   &       0.197   &      0.054   &       0.199   &       0.188   &      0.048   \\
                    &     (0.137)   &     (0.146)   &    (0.033)   &     (0.142)   &     (0.154)   &    (0.034)   \\
                    &               &               &               &               &               &               \\
IDR                 &    -0.004   	&    -0.003   	&   -0.001   	&    -0.002		&   -0.001   	&   -0.001   \\
                    &   (0.006)   	&   (0.006)   	&   (0.001)   	&   (0.006)   	&   (0.006)   	&   (0.001)   \\
                    &               &               &               &               &               &               \\
Inst. order         &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Wave                &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
Exp. day            &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   &         Yes   \\
\midrule
Pseudo R-sq.        &        0.08   &        0.09   &               &        0.13   &        0.15   &               \\
Obs                 &         305   &         268   &         305   &         305   &         268   &         305   \\
LL                  &        -190   &        -166   &               &        -180   &        -155   &               \\
AIC                 &         419   &         370   &           .   &         399   &         350   &           .   \\
BIC                 &         489   &         438   &           .   &         474   &         422   &           .   \\

==> tab_summaryGROUPS.tex <==
     &      \multicolumn{3}{c}{Partner=Human} & \multicolumn{3}{c}{Partner=Robot} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
                    &        Mean&          St. Dev.&       Obs&        Mean&          St. Dev.&       Obs\\
                    \midrule
\textbf{Verbal stimulus condition} &            &            &            &            &            &            \\
\rule{0pt}{4ex}\textit{Outcome variables}&        &            &            &        &            &            \\
Cooperate (Stage 1) &       0.640&       0.483&          86&       0.736&       0.443&          91\\
Cooperate (Stage 2) &       0.737&       0.443&          76&       0.630&       0.486&          81\\
\rule{0pt}{4ex}\textit{Control variables}&        &            &            &        &            &            \\
Female              &       0.628&       0.486&          86&       0.769&       0.424&          91\\
Freshman            &       0.663&       0.476&          86&       0.857&       0.352&          91\\
Economics           &       0.302&       0.462&          86&       0.440&       0.499&          91\\
Test failed         &       0.151&       0.360&          86&       0.099&       0.300&          91\\
\midrule
\textbf{No stimulus condition} &            &            &            &            &            &            \\
\rule{0pt}{4ex}\textit{Outcome variables}&        &            &            &        &            &            \\
Cooperate (Stage 1) &       0.663&       0.476&          86&       0.650&       0.480&          80\\
Cooperate (Stage 2) &       0.558&       0.500&          77&       0.380&       0.489&          71\\
\rule{0pt}{4ex}\textit{Control variables}&        &            &            &        &            &            \\
Female              &       0.802&       0.401&          86&       0.575&       0.497&          80\\
Freshman            &       0.791&       0.409&          86&       0.800&       0.403&          80\\
Economics           &       0.395&       0.492&          86&       0.450&       0.501&          80\\
Test failed         &       0.186&       0.391&          86&       0.075&       0.265&          80\\

==> tab_summarySTIMULUS.tex <==
     &      \multicolumn{3}{c}{No stimulus condition} & \multicolumn{3}{c}{Dialog stimulus condition} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
                    &        Mean&          St. Dev.&       Obs&        Mean&          St. Dev.&       Obs\\
                    \midrule
\textbf{Partner=Robot} &            &            &            &            &            &            \\
\rule{0pt}{4ex}\textit{Outcome variables}&        &            &            &        &            &            \\
Cooperate (Stage 1) &       0.736&       0.443&          91&       0.650&       0.480&          80\\
Cooperate (Stage 2) &       0.630&       0.486&          81&       0.380&       0.489&          71\\
\rule{0pt}{4ex}\textit{Control variables}&        &            &            &        &            &            \\
Female              &       0.769&       0.424&          91&       0.575&       0.497&          80\\
Freshman            &       0.857&       0.352&          91&       0.800&       0.403&          80\\
Economics           &       0.440&       0.499&          91&       0.450&       0.501&          80\\
Test failed         &       0.099&       0.300&          91&       0.075&       0.265&          80\\
\midrule
\textbf{Partner=Human} &            &            &            &            &            &            \\
\rule{0pt}{4ex}\textit{Outcome variables}&        &            &            &        &            &            \\
Cooperate (Stage 1) &       0.640&       0.483&          86&       0.663&       0.476&          86\\
Cooperate (Stage 2) &       0.737&       0.443&          76&       0.558&       0.500&          77\\
\rule{0pt}{4ex}\textit{Control variables}&        &            &            &        &            &            \\
Female              &       0.628&       0.486&          86&       0.802&       0.401&          86\\
Freshman            &       0.663&       0.476&          86&       0.791&       0.409&          86\\
Economics           &       0.302&       0.462&          86&       0.395&       0.492&          86\\
Test failed         &       0.151&       0.360&          86&       0.186&       0.391&          86\\
\bottomrule
